Developing Compelling Safety Cases

This paper describes a method for creating compelling safety cases. The method seeks to help improve safety case practice in order to address the weaknesses identified in current practice, in particular confirmation bias, after-the-fact assurance and safety cases as a paperwork exercise. Rather than creating new notations and tools to address these issues, we contend that it is improvements in the safety case process that will make the most significant improvement to safety case practice. Our method builds upon established approaches and best practice to create an approach that will ensure safety cases are risk-focused, seek to identify ways in which the system may not be safe (rather than just assuming it is), drive safe design and operation of the system (influencing the system itself rather than just documenting what's there), are used to support decisions made throughout the life of the system, including system operation and change, and encourage developers and operators to think about and understand why their system is safe (and when it isn't). A simple example of an infusion pump system is used to illustrate how the new method is applied in practice.

==> sections/case.tex <==
\section{Case Study}
\label{sec:case}

This section will use the example from JSS to show how this is a better, more affective way of achieving their aim...



==> sections/conformance.tex <==
\section{Completing the Safety Case: Conformance Arguments}
\label{sec:conform}

The method introduced in this paper has dealt with a number of the different aspects that are expected to be considered within a safety case, namely the risk, confidence and operational arguments for the system. In order to provide a complete safety case for the system there is another aspect that should be considered and that is the issue of conformance (or compliance) with safety standards. Although a compelling safety case can be created based upon risk, confidence and operational arguments, there is often also a requirement to demonstrate that applicable standards are satisfied, and the safety case can provide a mechnaism for achieving this through the provision of a \textbf{\textit{conformance argument}}. 

\textcolor{red}{As described in [conformance args paper Graydon et.al.] a conformance argument is...}

\textcolor{red}{It is important to note that a conformance argument may not always be the most effective way of demonstrating that the requirements of standards are met...}

\textcolor{red}{For those requirements of the standard where a conformance argument is considered to be required there may often be arguments created as part of the risk or confidence arguments that are able to be used to demonstrate conformance, for example... }
Rather than recreate those arguments as part of conformance argument, the conformance argument should refer to those parts of the risk or confidence arguments that are relevant.

Where required, the conformance arguments should be developed alongside the other safety case arguments to ensure that any constraints on the argument strategies adopted eminating from conformance obligations are considered as the safety case is developed, rather than seeking to modify the arguments later to ensure conformance can be demonstrated. 
